Count2Multiply: Reliable In-Memory High-Radix Counting

Computing-in-memory (CIM) has been demonstrated across various memory technologies, ranging from memristive crossbars performing analog dot-product computations to large-scale digital bitwise operations in commodity DRAM and other proposed non-volative memory technologies. However, current CIM solutions face latency and reliability challenges. CIM fidelity lags considerably behind access fidelity. Furthermore, bulk-bitwise CIM, although highly parallelized, requires long latency for operations like multiplication and addition, due to their bit-serial computation. This paper presents Count2Multiply, a technology-agnostic digital CIM approach to perform multiplication, addition and other operations using high-radix, massively parallel counting enabled by CIM bulk-bitwise logic operations. Designed to meet fault tolerance requirements, Count2Multiply integrates traditional row-wise error correction codes, such as Hamming and BCH, to address the high error rates in existing CIM designs. We demonstrate Count2Multiply with a detailed application to CIM in conventional DRAM due to its ubiquity and high endurance. However, we note that the Count2Multiply architecture is compatible with other functionally complete CIM proposals. Compared to the state-of-the-art in-DRAM CIM method, Count2Multiply achieves up to 10x speedup, 8x higher GOPS/Watt, and 9.5x higher GOPS/area, while outperforming GPU for vector-matrix multiplications.

==> figures/FaultTolerance/ProtectionListing.tex <==
\lstset{%
  basicstyle       = \ttfamily\fontsize{6}{7}\selectfont,
  frame            = tb,    % draw frame at top and bottom of code block
  tabsize          = 1,     % tab space width
  numbers          = left,  % display line numbers on the left
  numberstyle      = \color{gray}\ttfamily\tiny,
  numbersep        = 1pt,
  framesep         = 2pt,   % expand outward
  framerule        = 1pt, % make thicker
  morecomment=[l][\color{Blue}\fontsize{5}{5}]{//},
  showstringspaces = false  % do not mark spaces in strings
}
\begin{lstlisting}[escapechar = ~, linewidth = 3.5cm, name=asdf, label={lst:protection}] 
AAP M,B10//T2=T3=m
AAP b,B8//DCC0=!b,T0=b
AAP C1,B9//DCC1=0,T1=1
AAP B14,!B//!B=!b|m
AAP B15,A//A=b&m
AAP M,B9//DCC0=DCC1=!m
AP B12//MAJ<T0,T2,DCC0>
AP B13//MAJ<T1,T3,DCC1>
AAP !B,B5//DCC0=B
AAP oldA,B2//T2=oldA
AAP C1,B1//T1=1
AAP B14,b//b=B|oldA
\end{lstlisting}
\begin{tikzpicture}[remember picture, overlay,
    every edge/.append style = { ->, thick, >=stealth,
                                  draw=gray, dashed, line width = 1pt},
    every node/.append style = { align = left,
                                 font = \scriptsize\ttfamily }]
  \node [above right = 0 and 2.7cm of pic cs:line-asdf-1-start](A) {}; %not sure what 0 is adding but it makes it work better
  \node [below right = 0 and 2.7cm of pic cs:line-asdf-5-start](B) {};
  \node [above right = 0 and 2.8cm of pic cs:line-asdf-6-start](C) {};
  \node [below right = 0 and 2.8cm of pic cs:line-asdf-8-start](D) {};
  \node [above right = 0 and 2.5cm of pic cs:line-asdf-9-start](E) {};
  \node [below right = 0 and 2.5cm of pic cs:line-asdf-12-start](F) {};  
  \node [right = 2.65cm of pic cs:line-asdf-12-start](G) {};  
  \draw[decorate,decoration={brace, amplitude = 2pt}] (A){}+(0,0) -- node[right, inner sep=0pt, outer sep = 4pt] {Compute\\Masked\\Values} (B); %also adding zero really seems to help here...
  \draw[decorate,decoration={brace, amplitude = 2pt}] (C){}+(0,0) -- node[right, inner sep = 0pt, outer sep=4 pt] {Protect\\Masking} (D);
  \draw[decorate,decoration={brace, amplitude = 2pt}] (E){}+(0,0) -- node[right, inner sep = 0pt, outer sep=4 pt] {Update \& \\Protect \\Bit Value} (F);

\end{tikzpicture} 

==> figures/motivation/JohnsonCounter_RadixVsError.tex <==
\begin{tikzpicture}[scale=0.8]
\centering
\begin{semilogxaxis}[
    legend columns=2,
    legend style = {font=\footnotesize},
    xlabel={Capacity of Counters},
    ylabel={Normalized RMSE},
    xmin=10e1, xmax=10e18,
    ymin=0, ymax=0.225,
    xtick={1e3, 1e5, 1e7, 1e9, 1e11, 1e13, 1e15, 1e17},
    ytick={0, 0.05, 0.10, 0.15, 0.20},
    yticklabels={0, 0.05, 0.10, 0.15, 0.20},
    legend pos=north east,
    ymajorgrids=false,
    grid style=dashed,
    height=2in,
    width = .95\columnwidth
]
%radix 2
\addplot[
    color=blind_safe_one_scheme_eight_colors,
    mark=square*,
    ]
    coordinates {
(256,0.21108635878876497)(512,0.1972846087516225)(1024,0.1853898058976486)(2048,0.1748739538277342)(4096,0.16756882906475054)(8192,0.1613509083807886)(16384,0.15550896289227928)(32768,0.1495805013906153)(65536,0.14492644551950618)(131072,0.13968030992999966)(262144,0.13648651560921768)(524288,0.13065161647466766)(1048576,0.12881718260664884)(2097152,0.1264876478057856)(4194304,0.12398647641090049)(8388608,0.12122063831817458)(16777216,0.1178948288872346)(33554432,0.11590977968068157)(67108864,0.11343316638382496)(134217728,0.11002637956955537)(268435456,0.10819657780183536)(1073741824,0.10576747047749681)(1073741824,0.10576747047749681)(4294967296,0.10198585703775004)(4294967296,0.10198585703775004)(8589934592,0.10118915238918487)(17179869184,0.09982204768860468)(34359738368,0.09764266055351888)(68719476736,0.09574676653599773)(137438953472,0.09568339454638558)(274877906944,0.09476973640158246)(549755813888,0.09280398278464096)(1099511627776,0.09114554051508783)(2199023255552,0.08931902111402114)(4398046511104,0.08899289480929366)(8796093022208,0.08858209903580228)(17592186044416,0.08679536890329503)(35184372088832,0.08747713542181676)(70368744177664,0.08601150684695534)(281474976710656,0.08290700473059308)(281474976710656,0.08290700473059308)(562949953421312,0.08385416731123295)(1125899906842624,0.0817374683826688)(2251799813685248,0.080568910129411)(4503599627370496,0.07972491161466261)(9007199254740992,0.07883023399595022)(18014398509481984,0.07748778530638747)(36028797018963968,0.0785794362643285)(72057594037927936,0.07864228581963985)
    };
%Radix 4
\addplot[
    color=blind_safe_two_scheme_eight_colors,
    mark=*,
    ]
    coordinates { 
(256,0.22762694185487606)(1024,0.20102439570056804)(1024,0.20102439570056804)(4096,0.1837217920427511)(4096,0.1837217920427511)(16384,0.1695065597079198)(16384,0.1695065597079198)(65536,0.1571035896811835)(65536,0.1571035896811835)(262144,0.1473332153078888)(262144,0.1473332153078888)(1048576,0.14098949484048134)(1048576,0.14098949484048134)(4194304,0.13465337147948042)(4194304,0.13465337147948042)(16777216,0.12897142029323524)(16777216,0.12897142029323524)(67108864,0.12323436032646021)(67108864,0.12323436032646021)(268435456,0.11979194084205519)(268435456,0.11979194084205519)(1073741824,0.11587648113783101)(1073741824,0.11587648113783101)(4294967296,0.11243411237640985)(4294967296,0.11243411237640985)(17179869184,0.10788512358246483)(17179869184,0.10788512358246483)(68719476736,0.10502405608101752)(68719476736,0.10502405608101752)(274877906944,0.1034313758856227)(274877906944,0.1034313758856227)(1099511627776,0.09936027146386653)(1099511627776,0.09936027146386653)(4398046511104,0.09737056710305365)(4398046511104,0.09737056710305365)(17592186044416,0.09450725142990385)(17592186044416,0.09450725142990385)(70368744177664,0.09354958076116511)(70368744177664,0.09354958076116511)(281474976710656,0.09052522434889161)(281474976710656,0.09052522434889161)(1125899906842624,0.08910853545921735)(1125899906842624,0.08910853545921735)(4503599627370496,0.08836379912377855)(4503599627370496,0.08836379912377855)(18014398509481984,0.08537350677137025)(18014398509481984,0.08537350677137025)(72057594037927936,0.08407033956279579)(72057594037927936,0.08407033956279579)
};
%Radix 6
\addplot[
    color=blind_safe_three_scheme_eight_colors,
    mark=triangle*,
    ]
    coordinates {
(1296,0.1569104773672459)(1296,0.1569104773672459)(1296,0.1569104773672459)(7776,0.13807296524853246)(7776,0.13807296524853246)(46656,0.12556539996464197)(46656,0.12556539996464197)(46656,0.12556539996464197)(279936,0.11908823808782194)(279936,0.11908823808782194)(279936,0.11908823808782194)(1679616,0.11034464929085357)(1679616,0.11034464929085357)(10077696,0.10333191353526665)(10077696,0.10333191353526665)(10077696,0.10333191353526665)(60466176,0.09687335835114512)(60466176,0.09687335835114512)(362797056,0.0937943185124383)(362797056,0.0937943185124383)(362797056,0.0937943185124383)(2176782336,0.08954639169089067)(2176782336,0.08954639169089067)(2176782336,0.08954639169089067)(13060694016,0.08689516947036385)(13060694016,0.08689516947036385)(78364164096,0.08220064535112925)(78364164096,0.08220064535112925)(78364164096,0.08220064535112925)(470184984576,0.07845973457327089)(470184984576,0.07845973457327089)(2821109907456,0.07981898108032093)(2821109907456,0.07981898108032093)(2821109907456,0.07981898108032093)(16926659444736,0.0755720512477237)(16926659444736,0.0755720512477237)(101559956668416,0.07286653085144204)(101559956668416,0.07286653085144204)(101559956668416,0.07286653085144204)(609359740010496,0.07149914346236991)(609359740010496,0.07149914346236991)(609359740010496,0.07149914346236991)(3656158440062976,0.07015856862017775)(3656158440062976,0.07015856862017775)(21936950640377856,0.06838870353547512)(21936950640377856,0.06838870353547512)(21936950640377856,0.06838870353547512)(131621703842267136,0.06643839609185188)(131621703842267136,0.06643839609185188)
};
%Radix 8
\addplot[
    color=blind_safe_four_scheme_eight_colors,
    mark=square*,
    ]
    coordinates {
(512,0.13794417186342606)(512,0.13794417186342606)(4096,0.1188568232114335)(4096,0.1188568232114335)(4096,0.1188568232114335)(32768,0.10523569172018266)(32768,0.10523569172018266)(32768,0.10523569172018266)(262144,0.09751261015198306)(262144,0.09751261015198306)(262144,0.09751261015198306)(2097152,0.08875544051620358)(2097152,0.08875544051620358)(16777216,0.08289420585869575)(16777216,0.08289420585869575)(16777216,0.08289420585869575)(16777216,0.08289420585869575)(134217728,0.07834456171319425)(134217728,0.07834456171319425)(1073741824,0.07082515385967156)(1073741824,0.07082515385967156)(1073741824,0.07082515385967156)(1073741824,0.07082515385967156)(8589934592,0.07106111509024841)(8589934592,0.07106111509024841)(8589934592,0.07106111509024841)(68719476736,0.06629524576726568)(68719476736,0.06629524576726568)(68719476736,0.06629524576726568)(549755813888,0.0640954340342466)(549755813888,0.0640954340342466)(549755813888,0.0640954340342466)(4398046511104,0.06297204110042114)(4398046511104,0.06297204110042114)(35184372088832,0.06159005113490102)(35184372088832,0.06159005113490102)(35184372088832,0.06159005113490102)(35184372088832,0.06159005113490102)(281474976710656,0.061887744421408444)(281474976710656,0.061887744421408444)(281474976710656,0.061887744421408444)(2251799813685248,0.057055106009811264)(2251799813685248,0.057055106009811264)(2251799813685248,0.057055106009811264)(18014398509481984,0.055961777857537406)(18014398509481984,0.055961777857537406)(144115188075855872,0.05556924864727534)(144115188075855872,0.05556924864727534)(144115188075855872,0.05556924864727534)
 };
%Radix 10
\addplot[
    color=blind_safe_five_scheme_eight_colors,
    mark=*,
    ]
    coordinates {
(1000,0.11103203272029202)(1000,0.11103203272029202)(10000,0.09325408254065877)(10000,0.09325408254065877)(10000,0.09325408254065877)(10000,0.09325408254065877)(100000,0.08631122270823766)(100000,0.08631122270823766)(100000,0.08631122270823766)(1000000,0.07961338188134681)(1000000,0.07961338188134681)(1000000,0.07961338188134681)(10000000,0.07490944701284731)(10000000,0.07490944701284731)(10000000,0.07490944701284731)(10000000,0.07490944701284731)(100000000,0.06892571422755844)(100000000,0.06892571422755844)(100000000,0.06892571422755844)(1000000000,0.06212655393010009)(1000000000,0.06212655393010009)(1000000000,0.06212655393010009)(10000000000,0.05958937097058647)(10000000000,0.05958937097058647)(10000000000,0.05958937097058647)(10000000000,0.05958937097058647)(100000000000,0.056697246299734744)(100000000000,0.056697246299734744)(100000000000,0.056697246299734744)(1000000000000,0.05377494190629192)(1000000000000,0.05377494190629192)(1000000000000,0.05377494190629192)(10000000000000,0.0542784892912053)(10000000000000,0.0542784892912053)(10000000000000,0.0542784892912053)(10000000000000,0.0542784892912053)(100000000000000,0.048641924857872644)(100000000000000,0.048641924857872644)(100000000000000,0.048641924857872644)(1000000000000000,0.048756494153894214)(1000000000000000,0.048756494153894214)(1000000000000000,0.048756494153894214)(10000000000000000,0.0496590133889027)(10000000000000000,0.0496590133889027)(10000000000000000,0.0496590133889027)(10000000000000000,0.0496590133889027)(100000000000000000,0.0469949275642406)(100000000000000000,0.0469949275642406)(100000000000000000,0.0469949275642406)
};
%Radix 12
\addplot[
    color=blind_safe_six_scheme_eight_colors,
    mark=triangle*,
    ]
    coordinates {
(1728,0.0962024501740219)(1728,0.0962024501740219)(1728,0.0962024501740219)(20736,0.08115834371728706)(20736,0.08115834371728706)(20736,0.08115834371728706)(20736,0.08115834371728706)(248832,0.07119382746121677)(248832,0.07119382746121677)(248832,0.07119382746121677)(2985984,0.06560039024550317)(2985984,0.06560039024550317)(2985984,0.06560039024550317)(2985984,0.06560039024550317)(35831808,0.061189724234202145)(35831808,0.061189724234202145)(35831808,0.061189724234202145)(35831808,0.061189724234202145)(429981696,0.058460386544245874)(429981696,0.058460386544245874)(429981696,0.058460386544245874)(5159780352,0.05119128464477265)(5159780352,0.05119128464477265)(5159780352,0.05119128464477265)(5159780352,0.05119128464477265)(61917364224,0.048178786739165896)(61917364224,0.048178786739165896)(61917364224,0.048178786739165896)(743008370688,0.049647529158700625)(743008370688,0.049647529158700625)(743008370688,0.049647529158700625)(743008370688,0.049647529158700625)(8916100448256,0.04488954156905155)(8916100448256,0.04488954156905155)(8916100448256,0.04488954156905155)(8916100448256,0.04488954156905155)(106993205379072,0.04657906925594914)(106993205379072,0.04657906925594914)(106993205379072,0.04657906925594914)(1283918464548864,0.03925545229963504)(1283918464548864,0.03925545229963504)(1283918464548864,0.03925545229963504)(1283918464548864,0.03925545229963504)(15407021574586368,0.04077155112285531)(15407021574586368,0.04077155112285531)(15407021574586368,0.04077155112285531)(184884258895036416,0.04196929186442724)(184884258895036416,0.04196929186442724)(184884258895036416,0.04196929186442724)
 };
%Radix 14
\addplot[
    color=blind_safe_seven_scheme_eight_colors,
    mark=square*,
    ]
    coordinates { 
(2744,0.07711781725734941)(2744,0.07711781725734941)(2744,0.07711781725734941)(2744,0.07711781725734941)(38416,0.06616736268930613)(38416,0.06616736268930613)(38416,0.06616736268930613)(38416,0.06616736268930613)(537824,0.05837613241512669)(537824,0.05837613241512669)(537824,0.05837613241512669)(537824,0.05837613241512669)(7529536,0.056980802542040694)(7529536,0.056980802542040694)(7529536,0.056980802542040694)(105413504,0.05254470865150097)(105413504,0.05254470865150097)(105413504,0.05254470865150097)(105413504,0.05254470865150097)(1475789056,0.04955533816248731)(1475789056,0.04955533816248731)(1475789056,0.04955533816248731)(1475789056,0.04955533816248731)(20661046784,0.04726345639384503)(20661046784,0.04726345639384503)(20661046784,0.04726345639384503)(20661046784,0.04726345639384503)(289254654976,0.044343519152594914)(289254654976,0.044343519152594914)(289254654976,0.044343519152594914)(289254654976,0.044343519152594914)(4049565169664,0.04238218211158446)(4049565169664,0.04238218211158446)(4049565169664,0.04238218211158446)(56693912375296,0.037698961124763924)(56693912375296,0.037698961124763924)(56693912375296,0.037698961124763924)(56693912375296,0.037698961124763924)(793714773254144,0.03918626091042486)(793714773254144,0.03918626091042486)(793714773254144,0.03918626091042486)(793714773254144,0.03918626091042486)(11112006825558016,0.037128517573042905)(11112006825558016,0.037128517573042905)(11112006825558016,0.037128517573042905)(11112006825558016,0.037128517573042905)(155568095557812224,0.036322152281909124)(155568095557812224,0.036322152281909124)(155568095557812224,0.036322152281909124)
};
%Radix 16
\addplot[
    color=blind_safe_eight_scheme_eight_colors,
    mark=*,
    ]
    coordinates {
(256,0.08654376436598286)(4096,0.07242213231671657)(4096,0.07242213231671657)(4096,0.07242213231671657)(4096,0.07242213231671657)(65536,0.0611238933358881)(65536,0.0611238933358881)(65536,0.0611238933358881)(65536,0.0611238933358881)(1048576,0.055008074437099014)(1048576,0.055008074437099014)(1048576,0.055008074437099014)(1048576,0.055008074437099014)(16777216,0.04868987433111965)(16777216,0.04868987433111965)(16777216,0.04868987433111965)(16777216,0.04868987433111965)(268435456,0.04630005859880157)(268435456,0.04630005859880157)(268435456,0.04630005859880157)(268435456,0.04630005859880157)(4294967296,0.043366891345297996)(4294967296,0.043366891345297996)(4294967296,0.043366891345297996)(4294967296,0.043366891345297996)(68719476736,0.04110368326785491)(68719476736,0.04110368326785491)(68719476736,0.04110368326785491)(68719476736,0.04110368326785491)(1099511627776,0.035217293420843156)(1099511627776,0.035217293420843156)(1099511627776,0.035217293420843156)(1099511627776,0.035217293420843156)(17592186044416,0.03744038494426255)(17592186044416,0.03744038494426255)(17592186044416,0.03744038494426255)(17592186044416,0.03744038494426255)(281474976710656,0.03607956048230029)(281474976710656,0.03607956048230029)(281474976710656,0.03607956048230029)(281474976710656,0.03607956048230029)(4503599627370496,0.03228719266560236)(4503599627370496,0.03228719266560236)(4503599627370496,0.03228719266560236)(4503599627370496,0.03228719266560236)(72057594037927936,0.03177943613230473)(72057594037927936,0.03177943613230473)(72057594037927936,0.03177943613230473)(72057594037927936,0.03177943613230473)
 };
\legend{radix 2, radix 4, radix 6, radix 8, radix 10, radix 12, radix 14, radix 16}
\end{semilogxaxis}
\end{tikzpicture}

==> figures/motivation/count-ops.tex <==
\begin{tikzpicture}[scale=0.8]
    \begin{axis}[
        axis y line*=left,
        xlabel=Radix,
        ylabel=Av. ops incr. per counter,
        xmin=0, xmax=32,
        ymin=0, ymax=2500,
        xtick={4,8,12,16,20,24,28,32},
        ytick={500, 1000, 1500, 2000,  2500},
        height=2in,
        width=.95\columnwidth,
        ]
    \addplot[smooth,mark=+,blue] plot coordinates {
        (2, 1390.2463799999998)(4, 538.5405)(6, 507.38016)(8, 469.03896000000003)(10, 395.51352)(12, 451.49640000000005)(14, 506.232)(16, 436.74753999999996)(18, 477.99338)(20, 518.46075)(22, 558.11536)(24, 596.7083)(26, 634.58994)(28, 671.7996999999999)(30, 707.84708)(32, 743.3074499999999)

    }; \label{plot_one}
%    \addlegendentry{DRAM}

    \addplot[smooth,color=red,mark=x]
        plot coordinates {
            (2, 2317.0773)(4, 1012.45614)(6, 1014.76032)(8, 974.15784)(10, 842.61576)(12, 979.662)(14, 1113.7104)(16, 971.27438)(18, 1072.25542)(20, 1171.33725)(22, 1268.444)(24, 1363.0073799999998)(26, 1455.82398)(28, 1546.9883)(30, 1635.37084)(32, 1722.29775)

        }; \label{plot_two}
%    \addlegendentry{RTM}
    \end{axis}
       \begin{axis}[
        legend style={font=\small},
        legend cell align=left,        % <---
        legend pos=north west,
        axis y line*=right,
        axis x line=none,
%        xlabel=Radix,
%        ylabel=Rows per counter,
        xmin=0, xmax=32,
        ymin=0, ymax=72,
%        xtick={none},
        ytick={8, 16, 24, 32, 40, 48, 56, 64, 72},        height=2in,
        width=.95\columnwidth
        ]
\addlegendimage{/pgfplots/refstyle=plot_one}\addlegendentry{DRAM}
\addlegendimage{/pgfplots/refstyle=plot_two}\addlegendentry{RTM}
    \addplot[smooth,color=olive,mark=o]
        plot coordinates {
        (2, 32)(4, 24)(6, 28)(8, 30)(10, 30)(12, 35)(14, 40)(16, 36)(18, 40)(20, 44)(22, 48)(24, 52)(26, 56)(28, 60)(30, 64)(32, 68)

        };
    \addlegendentry{Memory Rows}
    \end{axis}
    \end{tikzpicture}

